MorphMLP: An Efficient MLP-Like Backbone for Spatial-Temporal Representation Learning

Recently, MLP-Like networks have been revived for image recognition. However, whether it is possible to build a generic MLP-Like architecture on video domain has not been explored, due to complex spatial-temporal modeling with large computation burden. To fill this gap, we present an efficient self-attention free backbone, namely MorphMLP, which flexibly leverages the concise Fully-Connected (FC) layer for video representation learning. Specifically, a MorphMLP block consists of two key layers in sequence, i.e., MorphFC_s and MorphFC_t, for spatial and temporal modeling respectively. MorphFC_s can effectively capture core semantics in each frame, by progressive token interaction along both height and width dimensions. Alternatively, MorphFC_t can adaptively learn long-term dependency over frames, by temporal token aggregation on each spatial location. With such multi-dimension and multi-scale factorization, our MorphMLP block can achieve a great accuracy-computation balance. Finally, we evaluate our MorphMLP on a number of popular video benchmarks. Compared with the recent state-of-the-art models, MorphMLP significantly reduces computation but with better accuracy, e.g., MorphMLP-S only uses 50% GFLOPs of VideoSwin-T but achieves 0.9% top-1 improvement on Kinetics400, under ImageNet1K pretraining. MorphMLP-B only uses 43% GFLOPs of MViT-B but achieves 2.4% top-1 improvement on SSV2, even though MorphMLP-B is pretrained on ImageNet1K while MViT-B is pretrained on Kinetics400. Moreover, our method adapted to the image domain outperforms previous SOTA MLP-Like architectures. Code is available at https://github.com/MTLab/MorphMLP.

==> tab/sota_ssv1.tex <==
\begin{table}[t]
\caption{Comparisons with the state-of-the-art on Something-Something V1 \cite{sth}. Our MorphMLP achieves the best results. }

    \setlength{\tabcolsep}{10.0pt}
    \centering
    \resizebox{0.8\columnwidth}{!}{
	\begin{tabular}{l|l|l|l|cc}
        \Xhline{1.0pt}
		\multirow{2}*{Method} & \multirow{2}*{Pretrain} & \multirow{2}*{\#Frame} & \multirow{2}*{GFLOPs} & \multicolumn{2}{c}{SSV1}  \\
		 ~ & ~ & ~  & ~ & Top-1 & Top-5 \\
        \Xhline{0.7pt}
		I3D\cite{video_as}  &IN-1K+K400 & 32$\times$3$\times$2 & 918 & 41.6  &72.2  \\
		NLI3D\cite{video_as}   &IN-1K+K400 & 32$\times$3$\times$2 & 1008 & 44.4  &76.0 \\
		NLI3D+GCN\cite{video_as}   &IN-1K+K400 & 32$\times$3$\times$2 & 1818 &46.1   &76.8 \\
		TSN\cite{tsn}   &IN-1K & 8$\times$1$\times$1 & 33   & 19.7  &46.6    \\
		TSM\cite{tsm}   &IN-1K+K400 & 16$\times$1$\times$1 & 65   & 47.2  &77.1\\
% 		TAM\cite{more_is_less}  &IN-1K &  16$\times$1$\times$2 & 95 & 48.4   &78.8 \\
% 		TANet\cite{tam}   &IN-1K &  16$\times$1$\times$1 & 66  & 47.6  &77.7 \\
		SmallBig\cite{smallbig}   &IN-1K & 16$\times$1$\times$1  &105   &49.3   &79.5 \\
		TEINet\cite{tei}   &IN-1K & 16$\times$3$\times$10 & 1980 & 51.0  &-  \\
		TEA\cite{tea}   &IN-1K & 16$\times$3$\times$10 & 2100 & 52.3  & 81.9  \\
		CT-NET\cite{ct_net}   &IN-1K & 16$\times$3$\times$2 & 447 & 53.4  & 81.7  \\
        \Xhline{0.7pt}
		MorphMLP-S & IN-1K  & 16$\times$1$\times$1 & 67  & 50.6 &78.0  \\
		MorphMLP-S & IN-1K  & 16$\times$3$\times$1 & 201  & 53.9 & 81.3  \\
		MorphMLP-B & IN-1K  & 16$\times$3$\times$1 & 294  & 55.5 &82.4  \\
		MorphMLP-B & IN-1K  & 32$\times$3$\times$1 & 591  & \textbf{57.4} &\textbf{84.5}  \\
    \Xhline{1.0pt}
	\end{tabular}
    }
    \label{sota_sthv1}

\end{table}  

